The Role of Gender in Social Network Organization

The digital traces we leave behind when engaging with the modern world offer an interesting lens through which we study behavioral patterns as expression of gender. Although gender differentiation has been observed in a number of settings, the majority of studies focus on a single data stream in isolation. Here we use a dataset of high resolution data collected using mobile phones, as well as detailed questionnaires, to study gender differences in a large cohort. We consider mobility behavior and individual personality traits among a group of more than $800$ university students. We also investigate interactions among them expressed via person-to-person contacts, interactions on online social networks, and telecommunication. Thus, we are able to study the differences between male and female behavior captured through a multitude of channels for a single cohort. We find that while the two genders are similar in a number of aspects, there are robust deviations that include multiple facets of social interactions, suggesting the existence of inherent behavioral differences. Finally, we quantify how aspects of an individual's characteristics and social behavior reveals their gender by posing it as a classification problem. We ask: How well can we distinguish between male and female study participants based on behavior alone? Which behavioral features are most predictive?

==> sections/author_summary.tex <==
Blablabla summary.

==> sections/related_work.tex <==
\paragraph{Genders and personality.}
The Big Five Inventory (BFI) is a widely used method for assessing human personality using 5 broad factors: Openness, Extraversion, Neuroticism, Agreeableness, and Conscientiousness \cite{john1999big}. 
Studies have repeatedly shown that women are more neurotic~\cite{costa2001gender,schmitt2007geographic,schmitt2008can,feingold1994gender} and agreeable~\cite{costa2001gender,williams1999pancultural,schmitt2007geographic,rubinstein2005big} than men. 
The gender differences in other traits from the big five are not so strongly pronounced and, perhaps, context specific.
Some studies report higher conscientiousness among women~\cite{rubinstein2005big} while others find men as more conscientious~\cite{williams1999pancultural}.
%A study carried out in 26 cultures using both college-age and adult samples showed that women consistently reported to be higher in Neuroticism, Agreeableness, and Openness to Feelings, whereas men were higher in Openness to Ideas \cite{costa2001gender}. Gender differences were more pronounced in Europe and USA, which was interpreted as a result of the individualistic values of the Western nations. Another cross-cultural research found that men scored higher in Extraversion, Conscientiousness, and Openness, while women's scores were higher for Agreeableness \cite{williams1999pancultural}. Even more studies have recorded greater Neuroticism \cite{schmitt2007geographic}, \cite{schmitt2008can}, \cite{feingold1994gender} and Agreeableness \cite{schmitt2007geographic}, \cite{budaev1999sex} for women. Moreover, a study conducted at a university in Israel found that female students were significantly more agreeable and conscientious than male students, regardless of the field of their study \cite{rubinstein2005big}.

Regarding self-esteem, Morris Rosenberg has defined it as a feeling of self-worth and proposed a 10-item instrument to measure it, which includes positive statements such as ``I feel that I have a number of good qualities'' and a number of negative propositions such as  ``I certainly feel useless at times'' \cite{rosenberg1965society}. Feingold \cite{feingold1994gender} found that males have slightly higher self-esteem than females, and Kling et al. \cite{kling1999gender} showed that this effect increases considerably in late adolescence. However, the literature is not consistent. There are observations that do not differentiate men from women with respect to self-esteem \cite{maccoby1974psychology}. An explanation for the existence of a difference is that men and women differ in their self-concepts, because they differ in the societal requirements that must be met to become ``good'' members of their respective gender \cite{cross1997models}. More precisely, men's self-esteem  emphasizes on one's personal distinguishing achievements, whereas women's self-esteem stems from connections and attachments to important others \cite{josephs1992gender}.

Self-esteem has been previously found to be positively correlated with narcissism \cite{twenge2003isn,emmons1984factor}. The latter involves a grandiose view of the self, a strong sense of entitlement and superiority, as well as tendencies to show dominant, charming, bragging, and aggressive behavior \cite{back2013narcissistic}. It can be assessed with the Narcisistic Admiration and Rivalry Questionnaire (NARQ), a 18-item instrument, which integrates two distinct cognitive and behavioral aspects of narcissism: the tendency to approach social admiration through self-enhancement, and the tendency for an antagonistic self-defense (rivalry) \cite{back2013narcissistic}. The literature here is consistent: men are more narcissistic than women, regardless the age and income \cite{grijalva2015gender,foster2003individual,bushman1998threatened,farwell1998narcissistic}. Like self-esteem, it is possible that a difference between the genders in narcissism is a consequence of the difference in self-construals with males being more individualistic and thus also more narcissistic.  

Several studies have been conducted to measure stress levels among students in higher education, reporting that female students tend to have more stress (and more stressors) than male students. This difference in stress levels is not solely derived from different initiators, but it can also be influenced by different control techniques. A study held among medical and law students found that factors such as deadlines, shortage of time, sexism and difficulties with partner were particularly stressful for the female students compared to male students \cite{clark1986gender}. Dahlin et al. \cite{dahlin2005stress} showed that female medical students rated stress factors that concerned negative expectations higher. Misra et al. \cite{misra2000academic} argued that higher levels of stress among women indicate that the latter ``like to compete, be noticed, loved, and worry for others, sometimes seeking perfect solutions that lead to higher anxiety and stress''. Finally, a study suggests that male students are less stressed because, among others, they benefit more from leisure activities \cite{misra2000college}. Although the aforementioned studies use different psychological instruments to measure stress, the results consistently demonstrate that women experience more stress than men. In this study, we measure stress with the widely used Perceived Stress Scale (PSS), which consists of 10 questions related to current level of experienced stress \cite{cohen1983global}.

Locus of control reflects the extent to which a person perceives a reward or reinforcement as contingent on his own behavior (internal locus) or as dependent on chance or environmental control (extrernal locus) \cite{rotter1966generalized}. It is measured with the 29-item I-E Rotter Scale, which consists of pairs of statements that a subject has to choose from. A lower score corresponds to internal locus, whereas a higher score indicates external locus. The two genders generally do not differ in this psychological principle \cite{rotter1966generalized,schultz2016theories,de1990sex,feingold1994gender}. However, women have responded differently in items related to academic achievements, favoring external control \cite{strickland1980sex}. Lefcourt \cite{lefcourt2013research} stated that those who are classified as internals not only perceive but also desire more personal control than externals and additionally found a significant gender effect for desired internal control in that females desired greater internal control than males.

Satisfaction with life constitutes a judgment of one's life in which the criteria for judgment are up to the person \cite{pavot1993review}. The Satisfaction with Life Scale (SWLS) instrument has been widely used to assess subjective well-being within various groups of population. It includes 5 generic statements such as ``In most ways my life is close to my ideal'', in which a subject must respond with a 1-7 scale, indicating the degree of agreement or disagreement. When gender is studied, the results are highly dependent on age. Within adolescents and elders, males have higher life satisfaction than females, while no observable difference is found among young adults \cite{neto1993satisfaction,pavot1991further}. 

Feelings of loneliness can be measured with UCLA, a 20-item scale, in which a subject must indicate how often an item is descriptive of him \cite{russell1996ucla}. Regarding gender-related differences in loneliness, male college students have been found to be more lonely than female students \cite{russell1996ucla,wiseman1995gender}. However, the outstanding differentiation between the genders, reported in the literature, is that men are less willing to acknowledge feelings of loneliness \cite{borys1985gender,cramer1998sex}, because the negative consequences of admitting loneliness are more for them.

Overall, women score higher in negative emotionality (such as neuroticism and stress) than men, but that may be due to their ease to admit or perceive such intense feelings. The presence of individualism also plays an important role in personality differences between the two genders. In the present study, we analyze the gender effect on the aforementioned personality traits in an environment where females are the numerical minority. The diverse dataset allows to unite the results from the questionnaires with the participants' behavior in natural settings.

\paragraph{Genders and mobility.}
Law \cite{law1999beyond} argues that daily mobility is admittedly not ``neutral'' and women's patterns in urban space are distinguishable from those of men. 
%He proposes an analytic framework that encloses the distinct aspects of gender, and their consequences in daily mobility. 
%These aspects include: a) a gender division of paid employment and non-work activities, b) gendered access to resources, such as time, money, technology, and skills, c) gendered experience of embodiment (e.g. physical deviations between men and women result to different experience of movement), d) the facets of masculinity and femininity (e.g. traditional stereotypes associate male and female with work and home respectively).
The frequency of trips is assumed to be similar between men and women, but the distance traveled and the mode of transportation varies.
Specifically, surveys conducted in Western countries in the '90s have demonstrated that women travel less kilometers than men and make more trips by walking or public transport \cite{polk1996swedish,rosenbloom2000trends}. 
Moreover, the purpose of traveling differs, with women traveling most frequently for household errands and men making the most trips to work. 
Other studies explain the shorter commuting distances of women as a result of their weaker position in the labor market \cite{camstra1996commuting}. 
Interestingly, females are observed to travel longer distances and explore larger areas in foraging tribes, which is argued to originate from the different expected return between hunting and collection \cite{hanson1980gender}. 

On the other hand, recent studies using mobile phone records have not observed any substantial differences in travel distances \cite{kang2010analyzing}, regularity, and predictability of movements \cite{song2010limits} between male and female commuters. 
However, when targeting to a specific group, a study using travel diary data collected in Portland, reports higher levels of activity among part-time employed women than those of part-time employed men throughout the day \cite{kwan2000interactive}.

In conclusion, even though in the last years researchers have been able to study mobility behavior of humans in detail by analyzing high resolution observational data, gender-based differences are rarely captured. This could mean that mobility patterns of women have changed through the years and the gap between the two genders found in earlier literature has been narrowed or that more research needs to be carried out in computational social science to reveal potential deviations.  For that, here we study the  mobility of men and women in an extensive range of aspects.  

\paragraph{Genders and social network organization.}
Previous studies show that the sizes of offline ego networks of the two genders are similar~\cite{caldwell1982sex,dunbar1995social,miritello2013limited}. 
On the other hand, women tend to have more friends online, for example in multiplayer games~\cite{szell2013women} and social networking services~\cite{acar2008antecedents,sheldon2008relationship,thelwall2008social}.

Men and women form social networks with high gender homophily, both offline~\cite{brass1985men} and online~\cite{laniado2016gender,thelwall2008social}.
Homophily has been studied as a function of transitivity (property according to which two individuals connected to a mutual alter are more likely to be connected themselves)~\cite{wasserman1994social}. 
On one hand, homophily is found to be strongly mitigated when pairs are already socially proximate (by sharing mutual acquaintances), where the degree of mitigation increases with increasing proximity~\cite{kossinets2009origins}. 
In contrast, Louch~\cite{louch2000personal} suggests that there are some empirical grounds for associating increased homophily with transitivity. 
However, the results of his study on gender homophily are contradictory; he finds that two neighbors of the same sex are significantly less likely to form ties than neighbors of the opposite sex. 
He additionally notes that transitivity increases with marriage, but less so if the alters are of the same gender, especially for men. 
Finally, a study in several schools in USA reports that females form more triads than males and that dyads consisting of females are more likely to be in triangles \cite{goodreau2009birds}. 
\todo{The part on homophily as a function on transitivity needs to be clearer}
% However, network size is found to be strongly dependent on age, marital status and employment of individuals. Unmarried young men and women do not differ in their number of friends, but this pattern changes after marriage, with married men reporting higher degree of social ties. 
% On the other hand, the numbers reverse for older adults, where women are found to have significantly more friends than men \cite{miritello2013limited}.

% Personal networks of men and women often differ in composition, with women's more focused on family and men's on nonkin, especially coworkers \cite{dunbar1995social}. 
% However, this difference disappears when age is controlled. Structural constraints on the development of social ties outside the family, such as childcare and domestic work, are experienced more often by women \cite{moore1990structural}. These findings suggest that men benefit more from the diverse networks and their weak ties with associates, which help them widen their career perspectives and increase their mobility in a professional environment. Men and women at work appear to build informal networks equally well, . In addition, even though in total women employees are found to be equally or more central, men appear to gain greater network returns from similar individuals and positional resources \cite{ibarra1992homophily}.

% \section{Gender Homophily, Transitivity, and Tie Dissolution}

% This tendency of individuals to form relationships with similar others has widely been documented in the literature as homophily. The conceptual idea of homophily can be traced back to Ancient Greece in the words of Plato (``similarity begets friendship'') and Aristotle (``we feel friendly towards those who are like ourselves in character and have similar desires'').  McPherson et al. \cite{mcpherson2001birds} have distinguished homophily into value homophily and status homophily. Value homophily is based on values, attitudes, and beliefs, whereas status homophily includes sociodemographic attributes like race, gender, or age, and acquired characteristics such as religion, education, or occupation. Their work also includes a review on gender homophily which starts as soon as children enter school with girls forming smaller, more homogeneous groups than boys. However, it is shown that this pattern fades as soon as adolescents move into romantic ties in puberty. 



==> sections/results.tex <==
\subsection*{Individual behavior}
To establish our findings related to social interactions, we start our analysis with the differences in individual aspects, namely the psychological dimensions and mobility patterns that distinguish men and women.
%Both areas have been intensively studied from a general point of view as well as with respect to gender differences \cite{costa2001gender}.

\subsubsection*{Personality}
For the personality analysis, we apply subsampling, and we test the null hypothesis that the two samples have equal means.
We start with the Big Five Inventory, and measure effect sizes between the two genders.
Figure~\ref{fig:effect-sizes-bfi} shows the normalized difference (i.e., the effect size) observed between males and females with respect to neuroticism, conscientiousness, agreeableness, extraversion and openness.
Each histogram represents the distribution of the difference in means normalized by the pooled standard deviation, when the mean in a subsample of females is substracted from the mean in a subsample of males (for details on the effect size, see.
Neuroticisim exhibits the largest deviation positioned far from the zero baseline on the negative side (with a mean of $d_\mathrm{neu}$=0.635), indicating that women score significantly higher in this personality characteristic than men. 
Significant alterations are found with respect to conscientiousness ($d_\mathrm{con} = 0.436$) and agreeableness ($d_\mathrm{agr} = 0.259$) as well, however, the differences are less profound.
On the other hand, there is no statistical significance in the average values of extraversion ($d_\mathrm{ext} = 0.118$) and openness ($d_\mathrm{ope} = 0.143$).
%
\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{figures/effect-sizes-bfi.pdf}
\caption{\textbf{Signed effect sizes of the BFI measured between men and woman.}
Negative values indicate that women achieve higher scores.
Histograms show the distribution of effect sizes defined by Eq.~(\ref{eq:effect_size}), horizontal bars denote 5 and 95\% percentiles. 
\label{fig:effect-sizes-bfi}}
\end{figure}
%
\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{figures/effect-sizes-personality.pdf}
\caption{\textbf{Signed effect sizes of personality traits measured between men and woman.}
Negative values indicate that women achieve higher scores.
Histograms show the distribution of effect sizes defined by Eq.~(\ref{eq:effect_size}), horizontal bars denote 5 and 95\% percentiles. 
\label{fig:effect-sizes-personality}}
\end{figure}
%
Figure.~\ref{fig:effect-sizes-personality} depicts the results on the other personality measures not included in the BFI.
Stress is significantly higher among women ($d_\mathrm{str} = -0.451$), while it is clear that men score higher in self-esteem ($d_\mathrm{se} = 0.423$).
Overall, narcissism is higher among male students ($d_\mathrm{nar} = 0.349$), but mainly due to rivalry ($d_\mathrm{riv} = 0.334$), which is its antagonistic aspect and less because of admiration ($d_\mathrm{adm} = 0.241$), which constitutes the assertive aspect of narcissism.
We find that women score higher in I-E Rotter Scale ($d_\mathrm{loc} = -0.157$), indicating a greater external locus of control.
They also score higher with respect to satisfaction with life ($d_\mathrm{sat} = -0.149$).
Finally, there is no statistically significant difference for loneliness ($d_\mathrm{lon} = 0.095$).

\subsubsection*{Mobility}
A common quantitative description of mobility behavior is by the distribution of unique locations visited by an individual in a time period, e.g., using $P_u(l)$, which is the relative frequency of visiting location $l$ by individual $u$~\cite{song2010limits,sekara2015fundamental}.
Relative frequency is estimated by the relative time the individual spent at the given location on a weekly basis.
Based on the GPS location collected in the CNS experiment, we first determine the labeled list of unique locations that characterize a user using the algorithm developed in Ref.~\cite{cuttone2014inferring}.

To further quantify one's mobility patterns, we measure the heterogeneity of the locations visited w.r.t time using entropy.
Entropy is a measure of uncertainty or predictability of a series, hereby used to capture the heterogeneity of individual visitation patterns:
\begin{equation}
H_u = -\sum_{l \in L(u)} P_u(l) \log P_u(l),
\end{equation}
where $L(u)$ denotes the set of locations for user $u$. 
Individuals distributing their time more evenly are characterized by higher entropy.
The effect sizes measured in the location related metrics are shown in Fig.~\ref{fig:effect-sizes-mobility}.
We find that women both visit more unique locations over time, and they have more homogeneous time distribution over their visited locations than me, indicating that time commitment of females is more widely spread across places.
%
\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{figures/effect-sizes-mobility.pdf}
\caption{\textbf{Effect sizes of the mobility indicators.}
Negative values indicate that women achieve higher scores.
Histograms show the distribution of effect sizes defined by Eq.~(\ref{eq:effect_size}), horizontal bars denote 5 and 95\% percentiles. 
\label{fig:effect-sizes-mobility}}
\end{figure}
%

\subsection*{Interactions}
Now we turn our attention towards social interactions among the students.
We consider three types of communication: physical proximity (i.e., person-to-person) interactions, Facebook activity, and mobile phone communication (calls and text messages).
Previous studies have shown that these channels describe social ties to a different extent as well as they form distinguished social environment resulting in different strength of links~\cite{sekara2014strength,onnela2007structure,eagle2009inferring,wilson2012review,wang2013showing}.
To corroborate this notion, in Fig.~\ref{fig:dyads} we report the fraction of active links in each communication channel.
Note that the vertical scale is logarithmic, indicating an increased presence of proximity links (purple pentagons), a moderate level of active Facebook connections (red circles) and a comparably low level of active telecommunication links (bottom curves).
%
\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{figures/dyads.pdf}
\caption{\textbf{Fraction of active dyads in the different networks.}
Curves show the number of active connections normalized by the total number of connections in the Facebook, telecommunication and physical proximity networks.\piotr{I think the month names are spelled with capital letters}
\label{fig:dyads}}
\end{figure}
%
We consider physical proximity networks as the weakest social interactions, due to the fact that in many social scenarios, for example university courses, an individual does not need to make significant effort in order to be in the proximity with others.
We assume that Facebook interactions represent a stronger relationship due to the more active actions it requires the students to create and maintain friendship with each other on the social network site.
Although users need to perform several tasks in order to make ties on Facebook, the actual communication between individuals is still considered low time-consuming \todo{REF}.
Finally, we assign the strongest social ties to phone calls and text messages based on the observation that both the creation and maintenance of mobile phone contacts correspond to the highest effort among the three channels and require the individuals to share a trusted relationship, as well as initiating and answering phone calls or text messages can be time-consuming \todo{REF}.
%
\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{figures/networks.pdf}
\caption{\textbf{A snapshot of the three interactions: (a) person-to-person, (b) Facebook feed and (c) phone call networks of the students obtained for a weekday (October 29, 2013).}
Blue and orange nodes correspond to male and female students respectively, link color denotes whether the connection is between the same genders.
The size of the nodes is proportional to their degree and width of the links represents the frequency of interactions.} 
\label{fig:networks}
\end{figure}
%
Figure~\ref{fig:networks} visualizes a daily snapshot of the three networks in this study.
The community structure revealed in the person-to-person network is a fingerprint of the classes the students attend together.
Less structure is observed in the Facebook feed network having a single large component, whereas the call network is the most fragmented of all of the networks.
Note the highl level of homophily in the proximity network (bold colored lines and colored cliques).
Clearly, the call network shows the highest fraction of mixed gender connections, a possible indicator of couples.
We explore the influence of gender homophily on formation of friendships in the various networks among the participants. 
To do this, we first identify the fraction of same-gender friends out of all friends an individual has.
Figure~\ref{fig:network_homophily} shows the $z$-scores of various network connections obtained by the comparison with the permutation model (see Methods).
Grey bar corresponds to the same gender connections.
Women have remarkably more same gender friends than the ones measured with the reference model in online interactions and phone communication. 
On the other hand, men also show a preference for forming homophilous ties through mobile communications, though to a less extent.
To study whether men and women tend to form triadic closures with same-gender alters, we count the various motifs in each network.
Results are shown in Fig.~\ref{fig:network_homophily} (color bars): male only (blue), female only (orange) and mixed (brown).
%
\begin{figure}[!ht]
\centering
\includegraphics[width=1\textwidth]{figures/network_homophily.pdf}
\caption{\textbf{Homophilous connection patterns in the three interaction networks.}
Bars represent the $z$-scores of connection motifs (containing two or three individuals) obtained from the comparison with the permutation model.
Grey color corresponds to dyadic connections, color bars denote triangles: male only (blue), female only (orange) and mixed (brown).
\label{fig:network_homophily}}
\end{figure}
%
Furthermore, we compare the results with the respective distribution of the expected motifs found in the reference model for the Facebook network (Figure \ref{fig:triangles}). 
We find that male-only triads are underrepresented compared to the reference model, and that there are more female-only motifs than what we would observed by chance.
Whereas a similar pattern is observed in person-to-person interactions, same-gender motifs are overrepresented for both genders in mobile communications.
It can be concluded that women prefer other women for both their dyadic and triadic relationships in every form of interaction, while homophily is noticeable among males only in their trusted interactions.
%
% \begin{table}[!ht]
% \centering
% \caption{
% {\bf Fraction of same-gender connections.}}
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \multicolumn{1}{l}{\bf } &\multicolumn{2}{|c}{\bf Males} & \multicolumn{2}{|c}{\bf Females}\\ \hline
% \multicolumn{1}{l}{\bf Network} & \multicolumn{1}{|l}{$Z$}  & \multicolumn{1}{l}{$r$} & \multicolumn{1}{|l}{$Z$}  & \multicolumn{1}{l}{$r$}\\
% \hline
% \multicolumn{1}{l}{\textit{ Facebook network}} & \multicolumn{1}{|c}{0.45}  & \multicolumn{1}{c}{1.02} & \multicolumn{1}{|c}{5.51} & \multicolumn{1}{c}{1.73}\\
% \multicolumn{1}{l}{\textit{ Calls network}} & \multicolumn{1}{|c}{2.68}  & \multicolumn{1}{c}{1.04} & \multicolumn{1}{|c}{7.09} & \multicolumn{1}{c}{1.75}\\
% \multicolumn{1}{l}{\textit{ Proximity network}} & \multicolumn{1}{|c}{0.58}  & \multicolumn{1}{c}{1.00} & \multicolumn{1}{|c}{1.33} & \multicolumn{1}{c}{1.06}\\
% \end{tabular}
% \begin{flushleft} \textit{Notes:} $Z$-scores and ratios $r$ relative to the reference model, estimated by Equations~(\ref{eq:zscore}) and~(\ref{eq:ratio}).
% \end{flushleft}
% \label{table-z}
% \end{table}
%


%This indicates that while there is an under-representation of male-only triads, triads solely consisting of females in the real network are significantly more than those obtained from the shuffled networks.
%
\begin{figure}[!ht]
\centering
\includegraphics[width=0.75\textwidth]{figures/triangles.pdf}
\caption{\textbf{Distributions of same-gender triangles in the Facebook friendship network.}
Empirical observations (black dashed lines) are compared to the distribution of triangles measured in the ensemble of null models.}
\label{fig:triangles}
\end{figure}
%

%
% \begin{table}[!ht]
% \centering
% \caption{
% {\bf Types of triangles in the networks}}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
% \multicolumn{1}{l}{\bf } &\multicolumn{2}{|c|}{\bf Facebook} & \multicolumn{2}{c|}{\bf Calls} & \multicolumn{2}{c}{\bf Proximity}\\ \hline
% \multicolumn{1}{l}{Type of triangles} &\multicolumn{1}{|c}{ $Z$} & \multicolumn{1}{c}{\bf $r$} &\multicolumn{1}{|c}{ $Z$} & \multicolumn{1}{c}{\bf $r$} &\multicolumn{1}{|c}{ $Z$} & \multicolumn{1}{c}{\bf $r$}\\ \hline
% \multicolumn{1}{l}{\bf Male-only} & \multicolumn{1}{|c}{-1.45}  & \multicolumn{1}{c}{0.91} & \multicolumn{1}{|c}{10.05}  & \multicolumn{1}{c}{1.59} & \multicolumn{1}{|c}{-2.77}  & \multicolumn{1}{c}{0.84}\\ 
% \multicolumn{1}{l}{\bf Female-only} & \multicolumn{1}{|c}{13.10}  & \multicolumn{1}{c}{3.98} & \multicolumn{1}{|c}{5.46}  & \multicolumn{1}{c}{3.35} & \multicolumn{1}{|c}{12.24}  & \multicolumn{1}{c}{3.62}\\
% \multicolumn{1}{l}{\bf Mixed-gender} & \multicolumn{1}{|c}{-0.53}  & \multicolumn{1}{c}{0.98} &
% \multicolumn{1}{|c}{-11.16}  & \multicolumn{1}{c}{0.46} & \multicolumn{1}{|c}{1.81}  & \multicolumn{1}{c}{1.09}\\
% \end{tabular}
% \begin{flushleft} \textit{Notes:} $Z$-scores and ratios $r$ relative to the reference model, estimated by Equations~(\ref{eq:zscore}) and~(\ref{eq:ratio}).
% \end{flushleft}
% \label{table-triads}
% \end{table}
%
Women are found to have significantly higher number of contacts than men in both online and mobile networks, whereas the size of the person-to-person networks are statistically the same.

Figure~\ref{fig:call-degree-trends} shows how degree varies with time in mobile communication (calls), with the females having more contacts for almost the entire period of interest.
\enys{we need to address  week 22}
\ioanna{Let me investigate the other networks as well. Also, I must have made a mistake with the ordering of the weeks in the graph: i.e. week 1 refers to 2014 but week 39 refers to 2013. I will update the file. UPDATE: I have added the new data files in the folder Weekly Degree. The lowest degrees correspond to the beginning of the experiment so it actually makes sense now.}
%
\begin{figure}[!ht]
\centering
\includegraphics[width=.69\textwidth]{figures/call-degree-trends.pdf}
\caption{\textbf{Degree of males and females per week in calls.}
Curves show the mean number of call contacts for males (blue) and females (orange).
\label{fig:call-degree-trends}}
\end{figure}
%
We measure betweenness centrality of each individual to investigate whether one gender is more prominently positioned in a network than the other.
We find that women consistently show higher betweenness indices, irrespective of the mode of interaction. 
In the literature, women are characterized by higher level of activity with respect to social media and phone, especially with their stronger ties.
To quantify predictability of the interactions, we calculate the entropy of the distribution of interactions over the contacts:
%
\begin{equation}
S_u = -\sum_{i \in N(u)} P_u(i) \log_2 P_u(i),
\label{contacts_entropy}
\end{equation}
%
where $P_u(i)$ is the probability that user $u$ interacts with their $i$-th contact in his ego-network $N(u)$.
The value of $S_u$ is estimated by the corresponding number of interactions relative to all interactions performed by user $u$.
Individuals who interact equally with many friends have high entropy (and therefore can be characterized by lower predictability), whereas those who limit the vast majority of their interactions to a small set of others are expected to have low entropy (more predictable).
In Fig.~\ref{fig:effect-sizes-network}, we plot the distribution of entropy effect sizes measured between males and females for the three interaction networks. 
Significant difference is observed for Facebook and calls, with women having higher entropy than men, indicating that females distribute their interactions with friends considerably more homogeneously.
In addition, females exchange remarkably more messages than men do ($p<.001$).
%
\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{figures/effect-sizes-network.pdf}
\caption{\textbf{Effect size distribution of network metrics.}
Negative values indicate that women achieve higher scores.
Histograms show the effect sizes of network related indicators (number of text messages and entropy) between males and females.
Horizontal bars denote the interval of 5 and 95\% percentiles.
\label{fig:effect-sizes-network}}
\end{figure}
%
With respect to time, women are described by significantly longer conversation times during phone calls than men are, regardless of the initiator of the call ($p<.0001$).
Longest calls are made from male to female (with an average duration of 117 seconds), with second longest calls observed between females (an average duration of 114.56 seconds). 
The shortest duration (71.52 seconds in average) is measured between males. 
%

% \begin{table}[!ht]
% \centering
% \caption{
% {\bf Call duration by pair}}
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \multicolumn{1}{l}{\bf } &\multicolumn{1}{|c}{\bf Males} & \multicolumn{1}{c}{\bf Females}\\ \hline
% \multicolumn{1}{l}{\bf Males} &
% \multicolumn{1}{|c}{71.52}  & \multicolumn{1}{c}{117.38}\\
% \multicolumn{1}{l}{\bf Females} &
% \multicolumn{1}{|c}{78.68 }  & \multicolumn{1}{c}{114.56}
% \end{tabular}
% \begin{flushleft} \textit{Note}: Rows indicate the genders of the party that initiated the call, columns indicate the receiver. Mean durations are in seconds. 
% \end{flushleft}
% \label{table_duration}
% \end{table}

%
\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{figures/effect-sizes-all.pdf}
\caption{\textbf{Summary of findings.}
Negative values indicate that women achieve higher scores.
Stripes show the 5 and 95\% percentile intervals of effect sizes over all indicators discussed in the paper.
Color corresponds to the type of indicators, and gray line marks the point of indifference.
\label{fig:ranking}}
\end{figure}

\subsection*{Gender prediction}
Based on the above results on observable quantities that differentiate between males and females, we consider the classification problem of predicting gender from individual and social characteristics.
The indicators revealing differences between genders are used as features to train four different models: \emph{logistic regressor}, \emph{AdaBoost}, \emph{support vector classifier} (SVC), \emph{random forest}, and \emph{gradient boosting classifier} implemented in the scikit-learn library~\cite{scikitlearn}.
The models are evaluated using 10-fold stratified cross-validation.
Each of the models underwent a hyperparameter fine tuning procedure described in detail in the Supplementary Information.

Men constitute 78\% of the study participants, which poses a significant imbalance in the data and therefore, we measure performance with the area under receiver operating characteristic curve (ROC-AUC) which is robust againts imbalance, as well as with the $F_1$ score that is sensitive to the imbalance.
The value of ROC-AUC can be interpreted as the probability that the classifier is able to identify a woman out of a pair of man and woman.
The $F_1$ score is the harmonic mean of precision (what fraction of people identified as women are actually women) and recall (what fraction of women are identified as women) at a selected threshold.

Results are summarized in Fig.~\ref{fig:model_performance} for each classifier along with the corresponding values of the random classifier based on the imbalance present in the data.
Logistic regression and gradient boosting classifier exhibit the highest performance both in terms of ROC-AUC and $F_1$ score, although the performance gain is slightly above the average.
\enys{Piotr: can you write some lines of what does it mean to have the same performance for all models?}
%
\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{figures/model_performance.pdf}
\caption{\textbf{Classifier performance in gender prediction.}
Reported are the ROC-AUC (black) and F$_\mathrm{1}$ (grey) scores for the five classifiers considered in the gender prediction.
Dashed lines mark the baseline obtained from the random classifer that takes the imbalance into account.
\label{fig:model_performance}}
\end{figure}

% <class 'sklearn.linear_model.logistic.LogisticRegression'>: AUC=0.87, F1=0.59, best_params: {'C': 1, 'n_jobs': 6}
% <class 'sklearn.ensemble.forest.RandomForestClassifier'>: AUC=0.86, F1=0.50, best_params: {'max_features': None, 'n_estimators': 1000, 'n_jobs': 7}
% <class 'sklearn.ensemble.gradient_boosting.GradientBoostingClassifier'>: AUC=0.87, F1=0.57, best_params: {'max_features': 'log2', 'n_estimators': 1000, 'learning_rate': 0.02}
% <class 'sklearn.ensemble.weight_boosting.AdaBoostClassifier'>: AUC=0.87, F1=0.57, best_params: {'n_estimators': 1000, 'learning_rate': 0.02}
% <class 'sklearn.svm.classes.SVC'>: AUC=0.86, F1=0.57, best_params: {'kernel': 'linear', 'C': 10, 'probability': True}

%
Next, we inspect the feature importance obtained by fitting a random forest to the data (Fig.~\ref{fig:feature-importance}).
We find that that gender homophily in the various networks (the fraction of male contacts) is among the most important features. 
Further important features include personality traits, such as neuroticism and narcissism, as well as specific network characteristics.
With respect to feature types, network indicators are the most important ones, occupying half of the top 6 indicators.
Features such as locus of control and stress promote personality traits to be the second most predictive, with BFI and mobility features showing the lowest average importance.
%
\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{figures/feature-importance.pdf}
\caption{\textbf{Feature importance obtained by Random Forest.}
Color shows the corresponding feature types: BFI (red), personality traits (green), mobility (yellow) and network (purple).
}
\label{fig:feature-importance}
\end{figure}



%


==> sections/si.tex <==

\subsection*{Personality traits}
We consider eleven personality traits in the main paper, with five traits forming the Big Five Inventory.
Table~\ref{tab:personality_traits} lists all the personality traits along with their definition and references to the corresponding literature.

\begin{table}[h]
\begin{tabular}{l|p{9cm}}
Personality trait & Description \\ \hline
Openness* &  Describes original, independent, creative and daring behavior \cite{schultz2016theories,goldberg1981language,digman1990personality,john1999big}. \\
Conscientiousness* & Desribes how careful, reliable, hardworking and organized is one \cite{schultz2016theories,goldberg1981language,digman1990personality,john1999big}. \\
Extraversion* & Sociable, talkative, fun-loving and affectionate \cite{schultz2016theories,goldberg1981language,digman1990personality,john1999big}. \\
Agreeableness* & Good-natured, softhearted, trusting and courteous \cite{schultz2016theories,goldberg1981language,digman1990personality,john1999big}. \\
Neuroticism* & Describes worried, insecure, nervous and highly strung state \cite{schultz2016theories,goldberg1981language,digman1990personality,john1999big}. \\
Self-esteem & A 10-item instrument to define the ``feeling of self-worth''. Example items are ``I feel that I have a number of good qualities'' and ``I certainly feel useless at times'' \cite{rosenberg1965society}. \\
Narcissism & A 18-item instrument (Narcisistic Admiration and Rivalry Questionnaire) describing a ``grandiose view of the self, a strong sense of entitlement and superiority, as well as tendencies to show dominant, charming, bragging, and aggressive behaviors'' \cite{back2013narcissistic}. \\
Perceived stress & A 14-item instrument (Perceived Stress Scale) that measures ``the degree to which situations in one's life are appraised as stressful'' \cite{cohen1983global}. \\
Locus of control & A 29-item instrument (I-E Rotter Scale) to measure ``the extent to which a person perceives a reward or reinforcement as contingent on his own behavior (internal locus) or as dependent on chance or environmental control (extrernal locus)'' \cite{rotter1966generalized,lefcourt2013research} \\
Satisfaction with life & A 5-item instrument (Satisfaction with life scale) that measures ``life satisfaction as a cognitive-judgmental process''. An example item is ``In most ways my life is close to my ideal'' \cite{diener1985satisfaction,pavot1993review}. \\
Loneliness & A 25-item instrument (UCLA Loneliness Scale) describing the ``perceived loneliness'' \cite{russel1978developing,russell1996ucla}. \\ \hline
\end{tabular}
\caption{Definition of the personality traits considered in this paper for the male and female freshmen students.
Traits marked with an asterisk (*) are part of the Big Five Inventory.
References provide further reading on the various personality traits.}
\label{tab:personality_traits}
\end{table}

